DESIL: Detecting Silent Bugs in MLIR Compiler Infrastructure

MLIR (Multi-Level Intermediate Representation) compiler infrastructure provides an efficient framework for introducing a new abstraction level for programming languages and domain-specific languages. It has attracted widespread attention in recent years and has been applied in various domains, such as deep learning compiler construction. Recently, several MLIR compiler fuzzing techniques, such as MLIRSmith and MLIRod, have been proposed. However, none of them can detect silent bugs, i.e., bugs that incorrectly optimize code silently. The difficulty in detecting silent bugs arises from two main aspects: (1) UB-Free Program Generation: Ensures the generated programs are free from undefined behaviors to suit the non-UB assumptions required by compiler optimizations. (2) Lowering Support: Converts the given MLIR program into an executable form, enabling execution result comparisons, and selects a suitable lowering path for the program to reduce redundant lowering pass and improve the efficiency of fuzzing. To address the above issues, we propose DESIL. DESIL enables silent bug detection by defining a set of UB-elimination rules based on the MLIR documentation and applying them to input programs to produce UB-free MLIR programs. To convert dialects in MLIR program into the executable form, DESIL designs a lowering path optimization strategy to convert the dialects in given MLIR program into executable form. Furthermore, DESIL incorporates the differential testing for silent bug detection. To achieve this, it introduces an operation-aware optimization recommendation strategy into the compilation process to generate diverse executable files. We applied DESIL to the latest revisions of the MLIR compiler infrastructure. It detected 23 silent bugs and 19 crash bugs, of which 12/14 have been confirmed or fixed

==> tables/pattern-back.tex <==



% \begin{table}[]
% \caption{Possible solution1 of fix pattern table.}
% \footnotesize
% \begin{tabular}{llll}
% \toprule
% \multicolumn{4}{c}{\normalsize \textbf{affine.vector\_store}}  \\
% \midrule
% Description & Example & UB Check & UB Prevension \\
% \begin{tabular}[c]{@{}p{2cm}@{}} Store a vector into a       memref with the given       position\end{tabular} & \begin{tabular}[c]{@{}l@{}}affine.vector\_store \\      \%v, \%m[\%idx0, \%idx1] : \\      memref<13x?xi16>, \\      vector<21xi16>\end{tabular} & \begin{tabular}[c]{@{}l@{}}For each $k \in [0, n)$, \\      Cond1: $\%idxk \in [0, dim(\%m, k)]$\\      Cond2: $(ElemNum(\%m) >= $  \\ $ ElemNum(\%v) +  $ \\ $     FlattenedPos(\%idx1, ..., \%idxn))$\end{tabular} & \begin{tabular}[c]{@{}p{5cm}@{}}1. Replace \%idxk with \%idxk         mod dim(\%m, k) if Cond1 holds.\\      2. Replace \%m with a new memref       value with enough space if Cond2 holds.\end{tabular} \\

% \bottomrule

% \end{tabular}
% \end{table}
\begin{table}[]
\caption{Fix patterns of undefined behaviors in scalar calculations.}
\scriptsize 
\begin{tabular}{@{}llll@{}}
\toprule

\multicolumn{4}{c}{\footnotesize \textbf{Shift Operations}}
\\
\midrule
Description & Example & Condition  & Prevention \\
\begin{tabular}[c]{@{}p{3cm}@{}}  Shift past bitwidth in shift operations, such as {\tt shri}.\end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  index.shrui \%1, \%2 \end{tabular} & 
\begin{tabular}[c]{@{}p{3cm}@{}}  1. The second operand (\%2 in the example) exceeds the bit width of the first operand (\%1 in the example).  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 holds, replace the second operand (\%2 in the example) with a random constant value within the bit width of the first operand (\%1 in the example). \end{tabular} \\

\midrule
\midrule





\multicolumn{4}{c}{\footnotesize \textbf{Signed Integer Division Operations}}                          
\\
\midrule
Description & Example & Condition  & Prevention \\
\begin{tabular}[c]{@{}p{3cm}@{}}  Signed division overflow and division by zero in signed division operations like {\tt divsi}. \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  index.divs \%1, \%2 \end{tabular} & 
\begin{tabular}[c]{@{}p{3cm}@{}}  1. The second operand (\%2 in example) is zero. \\ 2. The first operand (\%1 in example) is INT\_MIN (specific to its bitwidth), and the second operand (\%2 in example) is -1.  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 holds, replace the second operand (\%2 in exmaple) with nonzero random values. \\ If condition 2 holds, replace the second operand (\%2 in exmaple) with to non-(-1) random values. \end{tabular} \\


\midrule
\midrule


\multicolumn{4}{c}{\footnotesize \textbf{Unsigned Integer Division and Remainder Operations}}
\\
\midrule
Description & Example & Condition  & Prevention \\
\begin{tabular}[c]{@{}p{3cm}@{}}  Division by zero in unsigned integer division operations and remainder operations like {\tt divui} and {\tt remui}.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  index.divu \%1, \%2 \end{tabular} & 
\begin{tabular}[c]{@{}p{3cm}@{}}  1. The second operand (\%2 in example) is zero. \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 holds, replace the second operand (\%2 in example) with nonzero random signed or unsigned integer values (according to operand type). \end{tabular} \\







\bottomrule
\end{tabular}
\end{table}






\begin{table}[]
\caption{Fix patterns of index out-of-bounds undefined behaviors.}
\scriptsize 
\begin{tabular}{@{}llll@{}}
\toprule

\multicolumn{4}{c}{\footnotesize \textbf{Scalar Value Load and Store Operation}}
\\
\midrule
Description & Example & Condition  & Prevention \\
\begin{tabular}[c]{@{}p{3cm}@{}}  Out-of-bounds memory access in scalar load/store operations, such as {\tt memref.load}.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  affine.store \%0, \%m[\%idx1, \%idx2] : memref<13x?xi16> \end{tabular} & 
\begin{tabular}[c]{@{}p{3cm}@{}}  1. Any index (\%idx1, \%idx2 in the example) exceeds the size of the corresponding dimension of the array-like operand (\%m in the example).  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  Directly replace the old index operand with a new index value within the corresponding dimension size of the array-like operand using index.remu operation. \\ (e.g., replace \%idx1 with a new index within first dimension size of \%m, i.e., 13.) \end{tabular} \\


\midrule
\midrule


\multicolumn{4}{c}{\footnotesize \textbf{Dim Operations}}
\\
\midrule
Description & Example & Condition  & Prevention \\
\begin{tabular}[c]{@{}p{3cm}@{}}  Specified dimension index exceeds the rank in {\tt dim} operations.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  tensor.dim \%t, \%0 : tensor<?xi32>  \end{tabular} & 
\begin{tabular}[c]{@{}p{3cm}@{}}  1. The index value (\%0 in the example) exceeds the rank of array-like value (\%t in the example). \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 holds, replace old index operand (\%0 in example) with new index operand within the rank of array-like operand (\%t in example).  \end{tabular} \\






\midrule
\midrule





\multicolumn{4}{c}{\footnotesize \textbf{Array-Like Value Store and Load Operations}}   \\
\midrule
Description & Example & Condition & Prevention \\
\begin{tabular}[c]{@{}p{3cm}@{}}  Out-of-bounds memory access in array-like value store/load operations, such as {\tt affine.vector\_store}.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  affine.vector\_store \%o, \%c[\%idx0, \%idx1] : memref<13x?xi16>, vector<21xi16>  \end{tabular} & 
\begin{tabular}[c]{@{}p{3cm}@{}}  1. Any index operand (\%idx0, \%idx1 in example) exceeds the size of the corresponding dimensions of the data container operand (\%c in example). \\ 2. The remaining elements in the data container operand (\%c in example) are insufficient to store/load the data object operand (\%o in example) from the given starting position (\%idx0, \%idx1 in example).  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  Directly replace the index operand (\%idx0, \%idx1 in example) with a new index value within the corresponding dimension size of the data container operand using index.remu operation. \\ If condition 2 holds, replace the old data container operand (\%c in example) with a new data container that has sufficient elements.  \end{tabular} \\

\bottomrule
\end{tabular}
\end{table}








\begin{table}[]
\caption{Fix patterns of shape-related undefined behaviors-1.}
\scriptsize 
\begin{tabular}{@{}llll@{}}
\toprule

\multicolumn{4}{c}{\footnotesize \textbf{Yield Operations}}
\\
\midrule
Description & Example & Condition & Prevention \\
\begin{tabular}[c]{@{}p{2cm}@{}}  Shape inconsistency in yield operations.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  affine.for iter\_args(\%arg0=\%m) \\ affine.yield \%m1  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  1. The operand shape of the yield operation differs from the corresponding argument of the parent operation (e.g., the shape of \%m1 differs from \%m).  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 holds, replace the operand of the yield operation with another value that has the same shape as the corresponding argument of the parent operation.   \end{tabular} \\



\midrule
\midrule

\multicolumn{4}{c}{\footnotesize \textbf{linalg.broadcast}}
\\
\midrule
Description & Example & Condition & Prevention \\
\begin{tabular}[c]{@{}p{2cm}@{}}  Shape inconsistency in broadcast operation.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  linalg.broadcast ins (\%0 : tensor<?xi32>) outs (\%1 : tensor<?x64xi32>) dimensions=[1]  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  1. The shapes of the two operands (\%0 and \%1 in the example) are not same, except for the dimensions in {\tt dimensions}.  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 holds, replace the source operand (\%0 in the example) with a new tensor that has the same shape as the output operand (\%1 in the example), except for the size of dimensions in {\tt dimensions}.   \end{tabular} \\



\midrule
\midrule



\multicolumn{4}{c}{\footnotesize \textbf{linalg.generic}}
\\
\midrule
Description & Example & Condition & Prevention \\
\begin{tabular}[c]{@{}p{2cm}@{}}  Shape inconsistency in generic operation.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  linalg.generic { iterator\_types = ["parallel", "reduction"] } ins(\%1, \%2, \%3 : tensor<?x?xi1>, tensor<?x?xi1>, tensor<?x?xi1>) outs(\%4 : tensor<?xi1>) { region }  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  (Note that these conditions are specific to MLIRSmith-generated programs) \\ 1. The shapes of {\tt ins} operands (\%1, \%2, and \%3 in the example) are different. \\ 2. The dimension sizes of {\tt ins} operands (\%1, \%2, and \%3 in the example) specified as {\tt parallel} in {\tt iterator\_types} differ from the {\tt outs} operand (\%4 in the example). \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 or 2 holds, replace the {\tt ins} operands (\%1, \%2, and \%3 in the example) with tensors that have the same shape as the {\tt outs} operand (\%4 in the example), except for the size of dimensions marked as {\tt reduction} in {\tt iterator\_types}, and ensure that the shapes of the new tensors are the same.   \end{tabular} \\


\midrule
\midrule

\multicolumn{4}{c}{\footnotesize \textbf{linalg.matmul}}
\\
\midrule
Description & Example & Condition & Prevention \\
\begin{tabular}[c]{@{}p{2cm}@{}}  Shape inconsistency in matmul operation.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  linalg.matmul ins(\%1, \%2 : tensor<?x?xi64>, tensor<?x?xi64>) outs(\%3 : tensor<?x?xi64>) -> tensor<?x?xi64>  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  1. The second dimension of first {\tt ins} operand (\%1 in example) differs from the first dimension of second {\tt ins} operand (\%2 in example). \\ 2. The first dimension of first {\tt ins} operand (\%1 in example) differs from the first dimension of {\tt outs} operand (\%3 in example). \\ 3. The second dimension of second {\tt ins} operand (\%2 in example) differs from the second dimension of {\tt outs} operand (\%3 in example). \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If any 1-3 conditions hold, calculate the required dimension sizes for the {\tt ins} operands based on the {\tt outs} operand and replace the old {\tt ins} operands with new tensors, and ensure that the second dimension of the first {\tt ins} operand (\%1 in the example) matches the first dimension of the second {\tt ins} operand (\%2 in the example).   \end{tabular} \\

\midrule
\midrule

\multicolumn{4}{c}{\footnotesize \textbf{linalg.transpose}}
\\
\midrule
Description & Example & Condition & Prevention \\
\begin{tabular}[c]{@{}p{2cm}@{}}  Shape inconsistency in transpose operation.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  linalg.transpose ins (\%1 : tensor<?x?xi32>) outs (\%2 : tensor<?x?xi32>) permutation=[1, 0]  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  1. The dimension size of the {\tt ins} operand (\%1 in the example) differs from the corresponding dimension size of the {\tt outs} operand (\%2 in the example) as specified in {\tt permutation}. \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 holds, replace the {\tt ins} operand (\%1 in the example) with a new tensor that has the same corresponding dimension size as the {\tt outs} operand (\%2 in the example) as specified in {\tt permutation}.   \end{tabular} \\


\bottomrule
\end{tabular}
\end{table}








\begin{table}[]
\caption{Fix patterns of shape-related undefined behaviors-2.}
\scriptsize 
\begin{tabular}{@{}llll@{}}
\toprule


\multicolumn{4}{c}{\footnotesize \textbf{memref.cast and tensor.cast}}
\\
\midrule
Description & Example & Condition & Prevention \\
\begin{tabular}[c]{@{}p{3cm}@{}}  Shape inconsistency in cast operations.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  memref.cast \%m : memref<?x1xi32> to memref<10x?xi32>  \end{tabular} & 
\begin{tabular}[c]{@{}p{3cm}@{}}  1. When casting a dynamic dimension to static, the resulting static dimension size differs from the original static dimension size of the operand. \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 holds, for each dimension converted from dynamic to static, set the dimension size to match the corresponding original static dimension size of the operand.   \end{tabular} \\



\midrule
\midrule


\multicolumn{4}{c}{\footnotesize \textbf{Operations require operands with same shape.}}
\\
\midrule
Description & Example & Condition & Prevention \\
\begin{tabular}[c]{@{}p{3cm}@{}}  Shape inconsistency in copy operations and operations that perform arithmetic calculations on corresponding elements of two array-like values.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  linalg.copy ins(\%0 : tensor<?x?xi32>) outs(\%1 : tensor<?x?xi32>) -> tensor<?x?xi32>  \end{tabular} & 
\begin{tabular}[c]{@{}p{3cm}@{}}  1. The shapes of the two operands (\%0 and \%1 in the example) are not same.  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 holds, replace the source operand (\%0 in the example) with a new array-like value that has the same shape as the destination operand (\%1 in the example).   \end{tabular} \\



\bottomrule
\end{tabular}
\end{table}














\begin{table}[]
\caption{Fix patterns of other undefined behaviors. \cy{currently, memory-related undefined behaviors, because most of there kind of undefined behaviors are in memref dialect.}}
\scriptsize 
\begin{tabular}{@{}llll@{}}
\toprule


\multicolumn{4}{c}{\footnotesize \textbf{memref.assume\_alignment}}
\\
\midrule
Description & Example & Condition (static) & Prevention \\
\begin{tabular}[c]{@{}p{2cm}@{}}  Alignment information inconsistency in {\tt assume\_alignment} operation.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  memref. assume\_alignment \%m, 4 : memref<?x1xi32>  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  1. The alignment value (i.e., 4 in example) differs from the originally defined alignment information of the operand. \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 holds, replace the alignment information in this operation with the alignment information originally defined for the operand. If no such information is found, replace it with the default value defined in MLIR.   \end{tabular} \\


\midrule
\midrule


\multicolumn{4}{c}{\footnotesize \textbf{memref.realloc}}
\\
\midrule
Description & Example & Condition (static) & Prevention \\
\begin{tabular}[c]{@{}p{2cm}@{}}  Use the value after deprecated in {\tt realloc} operation.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  \%m1 = memref.realloc \%m0 : memref<64xi32> to memref<124xi32>  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  1. The original memref value is used after this operation. \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  If condition 1 holds, replace the usage of the original memref value after this operation with a new memref value.   \end{tabular} \\



\midrule
\midrule


\multicolumn{4}{c}{\footnotesize \textbf{Memory Allocation Operations}}
\\
\midrule
Description & Example & Condition (static) & Prevention \\
\begin{tabular}[c]{@{}p{2cm}@{}}  Uninitialized memory region.  \end{tabular} & 
\begin{tabular}[c]{@{}p{2cm}@{}}  \%0 = memref.alloca() : memref<1xi32>  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  Directly use the value in the result memref value without initialization is undefined behavior.  \end{tabular} & 
\begin{tabular}[c]{@{}p{4cm}@{}}  Initilize the content of memref value with linalg.fill.   \end{tabular} \\




\bottomrule
\end{tabular}
\end{table}
